Toroidal Hitomezashi Patterns

Extending a proposal of Defant and Kravitz [Discrete Mathematics, \textbf{1}, 347 (2024)], we define Hitomezashi patterns and loops on a torus and provide several structural results for such loops. For a given pattern, our main theorems give optimal residual information regarding the Hitomezashi loop length, loop count, as well as possible homology classes of such loops. Special attention is paid to toroidal Hitomezashi patterns that are symmetric with respect to the diagonal $x = y$, where we establish a novel connection between Hitomezashi and knot theory.

==> Figures/0011111.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[scale=.6]{Figures/0011111.png}
    \caption{The symmetric toroidal Hitomezashi pattern $\Cloth_{7,7}(x,x)$ for $x=--+++++$, with loops colored. The purple, orange, green loops are diagonal with homology $(1,1)$, while the rest four are null-homologous.}
    \label{fig:0011111}
\end{figure}
